Discovering Hidden Physics Behind Transport Dynamics

Transport processes are ubiquitous. They are, for example, at the heart of optical flow approaches; or of perfusion imaging, where blood transport is assessed, most commonly by injecting a tracer. An advection-diffusion equation is widely used to describe these transport phenomena. Our goal is estimating the underlying physics of advection-diffusion equations, expressed as velocity and diffusion tensor fields. We propose a learning framework (YETI) building on an auto-encoder structure between 2D and 3D image time-series, which incorporates the advection-diffusion model. To help with identifiability, we develop an advection-diffusion simulator which allows pre-training of our model by supervised learning using the velocity and diffusion tensor fields. Instead of directly learning these velocity and diffusion tensor fields, we introduce representations that assure incompressible flow and symmetric positive semi-definite diffusion fields and demonstrate the additional benefits of these representations on improving estimation accuracy. We further use transfer learning to apply YETI on a public brain magnetic resonance (MR) perfusion dataset of stroke patients and show its ability to successfully distinguish stroke lesions from normal brain regions via the estimated velocity and diffusion tensor fields.

==> sub/exp/fig/ixi_tab.tex <==
\begin{table}[t]
\hspace*{-0.325cm}
\resizebox{1.05\linewidth}{!}{
\centering
    \begin{tabular}{P{0.3cm}P{0.7cm}P{0.8cm}P{0.8cm}P{0.8cm}P{0.8cm}P{0.8cm}P{0.8cm}P{0.8cm}} 
    
       \toprule \\[-2.5ex]
        {\multirow{2}{*}{${ \mathbf N_{\text{in}}}$}}   &  {\multirow{2}{*}{{{\bf Mod.}}}}  &  {\multirow{2}{*}{\bf Conc.}} & \multicolumn{2}{c}{\bf Adv.-related}  & \multicolumn{4}{c}{\bf Diff.-related} \\%[-0.2ex] 
        \cmidrule(lr){4-5}
        \cmidrule(lr){6-9}
         &  &  & ${\mathbf{V}}$ & ${\|\mathbf{V}\|_2}$ & ${\mathbf{D}}$ & ${tr(\mathbf{D})}$ & FA & CbO \\ [-0.3ex]
         
     \midrule\\[-2ex]
       \parbox[t]{5mm}{\multirow{2}{*}{$5$}} &  {(a)}  &   &   &  & & & \\ [0.5ex]
        & {(b)}  &   &   &  & & &  \\ [0.5ex] 
       
     \hline\\[-2ex]
       \parbox[t]{5mm}{\multirow{2}{*}{$10$}} &  {(a)}  &   &   &  &  &  & \\ [0.5ex]
        & {(b)}  &   &   &  & & &  \\ [0.5ex] 
        
     \hline\\[-2ex]
       \parbox[t]{5mm}{\multirow{2}{*}{$15$}} &  {(a)}  &   &   &  &  &  & \\ [0.5ex]
        & {(b)}  &   &   &  & & &  \\ [0.5ex] 
        
     \hline\\[-2ex]
       \parbox[t]{5mm}{\multirow{2}{*}{$20$}} &  {(a)}  &   &   &  &  &  & \\ [0.5ex]
        & {(b)}  &   &   &  & & &  \\ [0.5ex] 

       
\midrule[\heavyrulewidth] \\ [-3ex]
\multicolumn{8}{l}{\footnotesize$^*$ Notations} \\ [-0.1ex]
\bottomrule
    \end{tabular}
}
\caption{Reconstruction errors comparison.}
    \label{tab: ixi}
\end{table}

==> sub/network/fig/pseudocode.tex <==

\begin{algorithm}[t]
\caption{Pseudocode for ... (See framework in Fig. \ref{fw})}
\label{algorithm}
{%\scriptsize
  \Input{Time series of concentration image patches $\{C_{\Omega_p}^{t_i} \in \mathbb{R}(\Omega_p) \vert\, i = 0,\, 1,\, \ldots,\, N_{\text{in}}\}$}
    \Output{Learned ${\bf{V}}$, ${\bf{D}}$, predicted concentrations $\{\widehat{C}_{\Omega_p}^{t_i} \in \mathbb{R}(\Omega_p) \vert\, i = 0,\, 1,\, \ldots,\, N_{\text{out}}\}$}
  %\Output{(a) Estimated velocity field ${\bf{V}}$ and diffusion field ${\bf{D}}$ \\ ~~~~~~~~~~~~ (b) Predicted CA concentration maps after $t_0$ with time interval $\delta t$}
 % \Settings{$\lambda_{\bf{V}},\, \sigma_{\bf{V}},\, \lambda_{\bf{D}},\, \sigma_{\bf{D}},\, k,\, \sigma$ in \Cref{eq: loss,eq: loss_cc,eq: ani_loss,eq: coef}, $\delta t$, $T_\text{pd}$, $lr$}
 % \Dataset{$S_i = \{ C^{t_j} \vert j = i,\, i+1,\, \ldots,\, i + T_\text{pd} \},\quad i = 0,\, 1,\, \ldots,\, T - T_\text{pd}$}
 % \Initialization{$\Gamma_1({\bf{x}}),\, \Gamma_2({\bf{x}}),\, L({\bf{x}}) \sim 0.001\times\mathcal{N}(0,\,1),\quad \forall {\bf{x}} \in \Omega$}

\tcc{Phase I: Physics Reconstruction}
\While{$\mathcal{L}_{I}$ not converged}   
   {
   Randomly pick time-course as training sample $S = \{C_{\Omega_p}^{t_j} \vert j = i,\, i+1,\, \ldots,\, i + N_\text{in} \}$ from $\{C_{\Omega_p}^{t_i}\}$  \label{2-1}\\  %\tcp*{Add comment} %,\quad i = 0,\, 1,\, \ldots,\, T - T_\text{pd}
   Reconstruct potentials $\boldsymbol{\Psi},\, \mathbf{B},\, \boldsymbol{\Lambda}$ (Sec.~\ref{sec: vd_net})  \label{2-2} \\
   Represent divergence-free $\mathbf{V}$ by $\boldsymbol{\Psi}$ via Eq.~(\ref{eq: repre_v})  \label{2-3} \\
   Represent symmetric PSD $\mathbf{D}$ by $ \mathbf{B},\, \boldsymbol{\Lambda}$ via Eq.~(\ref{eq: repre_psd})  \label{2-4} \\
   Compute $\mathcal{L}_{I}$ via Eq.~(\ref{eq: l1}) and backpropagate
   }
   
\tcc{Phase II: Longitudinal Regression}
\While{$\mathcal{L}_{II}$ not converged}   
   {
   Compute line \ref{2-1} - \ref{2-4}  \\
    \For{$t = t_i + \delta t,\, \ldots,\, t_{i+1},\, t_{i+1} + \delta t,\, \ldots,\, t_{i+N_{\text{out}}}$}
    { \label{time step}
   Discretize in space (Sec.\ref{sec: numerical})\\
   Compute advection-diffusion PDE via Eq.~(\ref{eq: adv_diff}) \\
   Impose patch-based virtual B.C. via Eq.~(\ref{eq: virtual_bc})\\
   Integrate in time (Sec.~\ref{sec: numerical}), obtain $\widehat{C}^{t+\delta t}$\\
   }
   %Predict concentration time-series: $\widehat{S}_{i} = \{ \widehat{C}^{t_j} \vert j = i,\, i+1,\, \ldots,\, i + T_\text{pd} \}$\\
   Compute $\mathcal{L}_{II}$ via Eq.~(\ref{eq: l2}) and backpropagate %(SGD with momentum)
   }}
\end{algorithm}
 

